Modelling Populations of Interaction Networks via Distance Metrics

Network data arises through observation of relational information between a collection of entities. Recent work in the literature has independently considered when (i) one observes a sample of networks, connectome data in neuroscience being a ubiquitous example, and (ii) the units of observation within a network are edges or paths, such as emails between people or a series of page visits to a website by a user, often referred to as interaction network data. The intersection of these two cases, however, is yet to be considered. In this paper, we propose a new Bayesian modelling framework to analyse such data. Given a practitioner-specified distance metric between observations, we define families of models through location and scale parameters, akin to a Gaussian distribution, with subsequent inference of model parameters providing reasoned statistical summaries for this non-standard data structure. To facilitate inference, we propose specialised Markov chain Monte Carlo (MCMC) schemes capable of sampling from doubly-intractable posterior distributions over discrete and multi-dimensional parameter spaces. Through simulation studies we confirm the efficacy of our methodology and inference scheme, whilst its application we illustrate via an example analysis of a location-based social network (LSBN) data set.

==> main/0-main.tex <==
\title{Modelling Populations of Interaction Networks via Distance Metrics}

\author{\name George Bolt \email g.bolt@lancaster.ac.uk\\
\addr STOR-i Centre for Doctoral Training\\
Lancaster University, Lancaster, UK, LA1 4YW
\AND
\name Sim\'{o}n Lunag\'{o}mez \email simon.lunagomez@itam.mx\\
\addr Department of Statistics\\
Instituto Tecnol\'{o}gico Aut\'{o}nomo de México (ITAM)\\
R\'{i}o Hondo 1, Altavista, Álvaro Obreg\'{o}n, 01080 Ciudad de M\'{e}xico, CDMX, Mexico
\AND
\name Christopher Nemeth \email c.nemeth@lancaster.ac.uk\\
\addr Department of Mathematics and Statistics\\
Lancaster University, Lancaster, UK, LA1 4YF
}

\ShortHeadings{Modelling Populations of Interaction Networks}{Bolt, Lunag\'{o}mez and Nemeth}

\editor{}

\maketitle


\begin{abstract}
  Network data arises through observation of relational information between a collection of entities. Recent work in the literature has independently considered when (i) one observes a sample of networks, connectome data in neuroscience being a ubiquitous example, and (ii) the units of observation within a network are edges or paths, such as emails between people or a series of page visits to a website by a user, often referred to as interaction network data. The intersection of these two cases, however, is yet to be considered. In this paper, we propose a new Bayesian modelling framework to analyse such data. Given a practitioner-specified distance metric between observations, we define families of models through location and scale parameters, akin to a Gaussian distribution, with subsequent inference of model parameters opening the door to reasoned statistical summaries for this non-standard data structure. To facilitate inference, we supplement this with specialised Markov Chain Monte Carlo (MCMC) algorithms capable of sampling from doubly-intractable posterior distributions over discrete and multi-dimensional parameter spaces. Through simulations studies we confirm the efficacy of our methodology and inference scheme, whilst its application we illustrate via an example analysis of a Location-Based Social Network (LSBN) data set. 
\end{abstract}


\begin{keywords}
  Interaction network, multiple networks, distance metrics, exchange algorithm, involutive MCMC.
\end{keywords}


\input{document/1-introduction}

\input{document/2-methods}

\input{document/3-model}

\input{document/4-inference}

\input{document/5-simulation_study}

\input{document/6-data_analysis}

\input{document/7-discussion}


\begin{appendices}

\appendix

\input{supplement/sample_spaces}
\input{supplement/simulations}

\begin{figure}
    \centering
    \includegraphics[page=2, width=0.85\linewidth]{img/data analysis/foursquare_analysis_main.pdf}
    \caption{Paths of our point estimate $\hat{\E}^m$ for the Foursquare data, alongside those of $\E^{(1)}$ and $\E^{(2)}$, its two nearest neighbours. The remaining paths can be seen in \Cref{fig:fsq_sim_est1,fig:fsq_sim_est3}.}
    \label{fig:fsq_sim_est2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[page=3, width=0.85\linewidth]{img/data analysis/foursquare_analysis_main.pdf} 
    \caption{Paths of our point estimate $\hat{\E}^m$ for the Foursquare data, alongside those of $\E^{(1)}$ and $\E^{(2)}$, its two nearest neighbours. The remaining paths can be seen in \Cref{fig:fsq_sim_est1,fig:fsq_sim_est2}.}
    \label{fig:fsq_sim_est3}
\end{figure}

\end{appendices}

\putbib
